Policy Evaluation in Continuous MDPs with Efficient Kernelized Gradient Temporal Difference

We consider policy evaluation in infinite-horizon discounted Markov decision problems (MDPs) with infinite spaces. We reformulate this task a compositional stochastic program with a function-valued decision variable that belongs to a reproducing kernel Hilbert space (RKHS). We approach this problem via a new functional generalization of stochastic quasi-gradient methods operating in tandem with stochastic sparse subspace projections. The result is an extension of gradient temporal difference learning that yields nonlinearly parameterized value function estimates of the solution to the Bellman evaluation equation. Our main contribution is a memory-efficient non-parametric stochastic method guaranteed to converge exactly to the Bellman fixed point with probability $1$ with attenuating step-sizes. Further, with constant step-sizes, we obtain mean convergence to a neighborhood and that the value function estimates have finite complexity. In the Mountain Car domain, we observe faster convergence to lower Bellman error solutions than existing approaches with a fraction of the required memory.

==> Algorithm.tex <==
%!TEX root = root.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%     S  E  C  T  I  O  N    %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace{-1.5mm}
\section{Functional Stochastic Quasi-Gradient}
\label{sec:algorithm}
%
%\subsection{}\label{subsec:quasi_fsgd}%\vspace{-2mm}
%
To apply functional SQG to \eqref{eq:main_prob}, {we} differentiate the compositional objective $L(V)$, which is of the form $L= g \circ h$, with $g(u)=\mathbb{E}_{\bbx, \pi(\bbx)} [(1/2) u^2]$ and $h(V) = \mathbb{E}_{\bby} [ r(\bbx, \pi(\bbx), \bby) + \gamma V(\bby) - V(\bbx) \given \bbx, \pi(\bbx)]$, and then consider its stochastic estimate. Consider the Frech$\acute{\text{e}}$t derivative of $L(V)$:%\vspace{-3mm}
%
\begin{align}\label{eq:grad}
\nabla_V \! L(V)
%&=\!\!\nabla_V \mathbb{E}_{\bbx, \!\pi(\bbx)}\!\big\{\!\frac{1}{2}\!( \mathbb{E}_{\bby}\![ r(\bbx,\!\pi(\!\bbx\!),\!\bby\!) \!\!+\! \gamma V\!(\bby\!) \! - \! \!V \!(\!\bbx) \!  \! \given\! \bbx, \!\pi(\!\bbx)])^2\!\big\} \! \nonumber\\
%
%&= \! \mathbb{E}_{\bbx, \!\pi(\bbx)}\!\big\{\!\nabla_V\!\frac{1}{2}\!( \mathbb{E}_{\bby}\![ r(\!\bbx,\!\pi(\!\bbx),\!\bby\!) \!\!+\! \gamma V\!(\bby\!) \! - \! \!V \!(\bbx\!) \! \!  \given\! \bbx, \!\pi(\!\bbx\!)])^2\!\big\} \! \nonumber\\
%
&=\mathbb{E}_{\bbx, \pi(\bbx)}\big\{ \mathbb{E}_{\bby} [ \gamma\kappa(\bby, \cdot) - \kappa(\bbx,\cdot)\given \bbx, \pi(\bbx)] \\
&\qquad\quad \times\mathbb{E}_{\bby}\![ r(\bbx,\!\pi(\bbx),\!\bby\!) \!\!+\! \gamma V\!(\bby\!) \! - \! \!V \!(\bbx) \!   \given\! \bbx, \!\pi(\bbx)]  \big\} \nonumber
\end{align}
%
Here we pull the differential operator inside the expectation and use both the chain rule and reproducing property of the kernel \eqref{eq:rkhs_properties}(i). %Now, we can use the law of total expectation to simplify the last line of \eqref{eq:grad} to 
%%
%\begin{align}\label{eq:grad2}
%\nabla_V J(V) =  \mathbb{E}_{\bbx, \pi(\bbx),\bby} \left[ \gamma\kappa(\bby, \cdot) - \kappa(\bbx,\cdot)\right] \mathbb{E}_{\bbx, \pi(\bbx),\bby}\left[ r(\bbx,\pi(\bbx),\bby) + \gamma V(\bby) -  V (\bbx)   \right]   
%\end{align}
%%
For future reference, we define the expression $\mathbb{E}_{\bby} [ r(\bbx, \pi(\bbx), \bby) + \gamma V(\bby) - V(\bbx) \given \bbx, \pi(\bbx)] = \bar{\delta}$ as the average temporal difference \cite{sutton1988learning}. To perform stochastic descent in function space $\ccalH$, we need a stochastic approximate of \eqref{eq:grad} evaluated at a state-action-state triple $(\bbx, \pi(\bbx), \bby)$, which together with the regularizer yields%\vspace{-1mm}
%
\begin{align}\label{eq:stoch_grad}
{\nabla}_V &J(V , \delta ; \bbx, \pi(\bbx), \bby)  \\
&= \!\left[ \gamma\kappa(\bby, \!\cdot) \!-\! \kappa(\bbx,\!\cdot)\right] \!
\left[ r(\bbx,\pi(\bbx),\bby)\! +\! \gamma V\!(\bby\!) \!- \!  V \!(\bbx\!)\!   \right] \!+\! \lambda V\nonumber
\end{align}
%
where $\delta := r(\bbx, \pi(\bbx), \bby) + \gamma V(\bby) - V(\bbx)$ is defined as the (instantaneous) temporal difference.
%
Observe that we cannot obtain samples of ${\nabla}_V J(V, \delta ; \bbx, \pi(\bbx), \bby)$ with a single query to a simulation oracle: stochastic gradient method would estimate one of the expected gradients by its instantaneous approximation, but would still leave a second expected value that depends on infinitely many realizations of either prior distribution and policy $(\bbx, \pi(\bbx))$ or MDP transition dynamics $\bby$, a problem first identified in \cite{sutton2009convergent} for finite MDPs where it is called the \emph{double sampling problem}. {Double sampling aside, an equally significant  challenge associated with using \eqref{eq:stoch_grad} as a candidate descent direction is that classically we would compute its expectation conditional on the algorithm history, but due to the dependence of the factors, this does not yield \eqref{eq:grad}. In particular, the stochastic gradient is \emph{biased} with respect to \eqref{eq:grad} due to the inner conditional expectation in \eqref{eq:grad}.}

 To mitigate these issues, we {require} a method {that constructs} a \emph{coupled} stochastic descent procedure by considering noisy estimates of both factors in the product-of-expectations expression in \eqref{eq:grad}. 
%
The first factor $\left[ \gamma\kappa(\bby, \cdot) - \kappa(\bbx,\cdot)\right] $ in \eqref{eq:stoch_grad} is a difference of kernel maps, so {estimating its expectation is parameterized by infinitely many samples of $\bbx$ and $\bby$ \cite{Kivinen2004,smola2007hilbert}.} Instead, we propose a sequence based on samples of the second scalar factor to estimate its expected value. Specifically, from samples of $\delta
$, consider a recursion $z_t$ that estimates $\bar{\delta}$ as
%
\begin{align}\label{eq:td_average}
&\delta_t = r(\bbx_t, \pi(\bbx_t), \bby_t) + \gamma V_t(\bby_t) - V_t(\bbx_t)  \nonumber\\
&z_{t+1} = (1-\beta_t) z_t + \beta_t \delta_t
\end{align}
%
where we define $\delta_t$ \cite{sutton1988learning} as the temporal difference at time $t$ in \eqref{eq:td_average}.
%
Thus, \eqref{eq:td_average} averages the TD sequence $\delta_t$: $z_t$ estimates $\bar{\delta}_t$, and $\beta_t\in (0,1)$ is a learning rate.

To define a stochastic descent step, we replace the first factor inside the outer expectation in \eqref{eq:grad} with its instantaneous approximate, {i.e., $ \left[ \gamma\kappa(\bby_t, \cdot) - \kappa(\bbx_t,\cdot)\right]$,} at sample $(\bbx_t, \pi(\bbx_t), \bby_t)$, which yields the stochastic quasi-gradient step %\vspace{-2mm}
%
\begin{equation}\label{eq:quasi_fsgd}
\hat{V}_{t+1} =(1-\alpha_t\lambda)\hat{V}_t - \alpha_t (\gamma \kappa(\bby_t, \cdot) - \kappa(\bbx_t,\cdot))z_{t+1}  \; .
\end{equation}
%
where the coefficient $(1-\alpha_t \lambda)$ comes from the regularizer, and $\alpha_t$ is a positive scalar learning rate. This update is a stochastic quasi-gradient step because the true stochastic gradient of $J(V)$ is $(\gamma \kappa(\bby_t, \cdot) - \kappa(\bbx_t,\cdot))\delta_{t}$, but this estimator is unavailable with a single trajectory of the MDP since the factors in this product are dependent. By replacing $\delta_t$ by auxiliary variable $z_{t+1}$ this issue may be circumvented in the construction of coupled supermartingales (Section \ref{sec:convergence}).

{\bf Kernel Parameterization} Suppose $V_0=0\in \ccalH$. Then, \eqref{eq:quasi_fsgd} at time $t$, making use of the Representer Theorem \eqref{eq:kernel_expansion}, implies the function $\tilde{V}_t$ is a kernel expansion of past states $(\bbx_t, \bby_t)$ as\vspace{-1mm}
%
\begin{align}\label{eq:kernel_expansion_t}
\hat{V}_t(\bbx) 
= \sum_{n=1}^{2(t-1)} w_n \kappa(\bbv_n, \bbx)
= \bbw_t^T\boldsymbol{\kappa}_{\bbX_t}(\bbx) \; .%%\vspace{-5mm}
\end{align}
%
On the right-hand side of \eqref{eq:kernel_expansion_t} we introduce the notation $\bbv_n = \bbx_{n/2} \text{ for } n \text{ even}$ and $\bbv_n = \bby_{n/2 + 1} \text{ for } n \text{ odd}$, and:
%
%\begin{align}\label{eq:stacking_notation}
%
$\bbw_t = [w_1, \cdots, w_{2(t-1)}] \in \reals^{2(t-1)} \; ,$ 
$\bbX_t = [\bbx_1, \bby_1, \ldots, \bbx_{t-1}, \bby_{t-1}]\in \reals^{p\times 2(t-1)} \; ,$
%
%\end{align}
%
and $\boldsymbol{\kappa}_{\bbX_t}(\cdot) = [\kappa(\bbx_1,\cdot),\ \kappa(\bby_1,\cdot), \ \ldots\ ,\kappa(\bbx_{t-1},\cdot), \kappa(\bby_{t-1},\cdot)]^T \; .$
 The kernel expansion in \eqref{eq:kernel_expansion_t}, together with the functional update \eqref{eq:quasi_fsgd}, yields the fact that functional SQG in $\ccalH$ amounts to the following updates on the {data matrix $\bbX$, henceforth referred to as a kernel dictionary,} and coefficient vector $\bbw$:%\vspace{-1mm}
%
\begin{align}\label{eq:param_update} 
&\bbX_{t+1} = [\bbX_t \; , \; \bbx_t \; , \; \bby_t] , \nonumber\\
&\bbw_{t+1} = [ (1 - \alpha_t \lambda) \bbw_t \; , \; \alpha_t z_{t+1} \; , \; -\alpha_t \gamma z_{t+1}]  \; ,
\end{align}
%
Observe that this update causes $\bbX_{t+1}$ to have two more columns than $\bbX_t$. We define the \emph{model order} as number of data points $M_t$ in the dictionary at time $t$, which for functional stochastic quasi-gradient descent is $M_t = 2(t-1)$. Asymptotically, then, the complexity of storing $\hat{V}_t(\bbx)$ is infinite. %We address this issue next, inspired by \cite{koppel2019parsimonious}.%\vspace{-2mm}

%
\subsection{Sparse Stochastic Subspace Projections}\label{subsec:polk_projection}%\vspace{-2mm}
%

%{(can this be shortened since we just identified the issue in the previous sentence?  perhaps ``Because of the infinite complexity associated with storing $\hat{V}_t(\bbx)$, ..."?) 
%
Since the update \eqref{eq:quasi_fsgd} has complexity $\ccalO(t)$ due to the RKHS parameterization \cite{Kivinen2004,koppel2019parsimonious}, it is impractical {in} settings with streaming data or arbitrarily large training sets. We address this issue by replacing the stochastic descent step \eqref{eq:quasi_fsgd} with an orthogonally projected variant \cite{koppel2019parsimonious}, where the projection is onto a low-dimensional functional subspace $\ccalH_{\bbD_{t+1}}$ of $\ccalH$, i.e.,%\vspace{-1mm}
%
\begin{align}\label{eq:quasi_projected_fsgd}
\!\!\!\!\!\!V_{t+1}\! \!=\!\ccalP_{\ccalH_{\bbD_{t+1}}}\![(1 \!-\! \alpha_t \lambda\!) V_t \!  -\! \alpha_t (\!\gamma \kappa(\bby_t, \!\cdot) \!-\! \kappa(\!\bbx_t,\cdot\!))z_{t+1}\! ]  ,
\end{align}
%
where $\alpha_t$ again is a scalar step-size, and $\ccalH_{\bbD_{t+1}}=\text{span}\{\kappa(\bbd_n, \cdot) \}_{n=1}^{M_t}$ for some collection of sample instances $\{\bbd_n\}\subset \{\bbx_u\}_{u\leq t}$. Note that the un-projected function SQG method \eqref{eq:quasi_fsgd} may be interpreted as conducting a sequence of orthogonal projections, which motivates the design of \eqref{eq:quasi_projected_fsgd}. Specifically, rewrite \eqref{eq:quasi_fsgd} as the quadratic minimization
%
\begin{align}\label{eq:proximal_hilbert_dictionary}
\hat{V}_{t+1} &\!\!=\! \argmin_{V \in \ccalH} \!
\Big\lVert  V \!\!\!-\! \!\Big(\!\!(\!1\!-\!\alpha_t \lambda\!)\! \hat{V}_t \!
\!-\! \alpha_t \!  (\!\gamma \kappa(\!\bby_t,\! \cdot\!) \!
 - \!\kappa(\!\bbx_t,\!\cdot\!)\!)z_{t+1}\!\! \Big)\!\Big\rVert_{\ccalH}^2 \nonumber \\
%
&\!\!=\!\! \argmin_{V \in \ccalH_{\bbX_{t+1}}}\!\! \!
\Big\lVert  V \!\!\!-\! \!\Big(\!\!(\!1\!-\!\alpha_t \lambda\!)\! \hat{V}_t \!
\!-\! \alpha_t \!  (\!\gamma \kappa(\!\bby_t,\! \cdot\!) \!
 - \!\kappa(\!\bbx_t,\!\cdot\!)\!)z_{t+1}\!\! \Big)\!\Big\rVert_{\ccalH}^2, 
\end{align}
%
where the first equality in \eqref{eq:proximal_hilbert_dictionary} comes from ignoring constant terms which vanish upon differentiation with respect to $V$, and the second comes from observing that $V_{t+1}$ can be represented using only the points $\bbX_{t+1}$, using \eqref{eq:param_update}.  Notice \eqref{eq:proximal_hilbert_dictionary} expresses $V_{t+1}$ as the projection $(1-\alpha_t \lambda) V_t 
- \alpha_t   (\gamma \kappa(\bby_t, \cdot) - \kappa(\bbx_t,\cdot))z_{t+1}$ onto the subspace defined by dictionary $\bbX_{t+1}$.

Rather than {selecting} dictionary $\bbD=\bbX_{t+1}$, we propose instead to select a different dictionary, $\bbD=\bbD_{t+1}$, which is extracted from the data points observed thus far, at each iteration.  {The process by which we select $\bbD_{t+1}$ is delayed for now, but is of dimension $p \times {M}_{t+1}$. We design a scheme such that  ${M}_{t+1}$ is \emph{independent} of $t$, and instead determined by fundamental topological properties of state space $\ccalX$, i.e., a generalization of the Nyquist rate \cite{zhou2002covering}.}  As a result, the sequence ${V}_t$ differs from the functional stochastic quasi-gradient method $\hat{V}_t$ presented at the outset of this section. %We {enforce} function parsimony by selecting dictionaries $\bbD$ that $M_t << \ccalO(t)$.

Specifically, suppose the function ${V}_{t+1}$ is parameterized dictionary $\bbD_{t+1}$ and weight vector $\bbw_{t+1}$. We denote columns of $\bbD_{t+1}$ as $\bbd_n$ for $n=1,\dots,{M}_{t+1}$, where the time index is dropped for notational clarity but may be inferred from the context.
%
Setting aside how $\bbD_{t+1}$ is chosen for now, we replace the update \eqref{eq:proximal_hilbert_dictionary} in which the dictionary grows at each iteration by the  functional stochastic quasi-gradient sequence projected onto the subspace $\ccalH_{\bbD_{t+1}}=\text{span}\{ \kappa(\bbd_n, \cdot) \}_{n=1}^{M_{t+1}}$ as\vspace{-2mm}
%
\begin{align}\label{eq:projection_hat}
{V}_{t+1}&\!=\!\! \argmin_{V \in \ccalH_{\bbD_{t+1}}}\!\! \!
\Big\lVert  V \!\!\!-\! \!\Big(\!\!(\!1\!-\!\alpha_t \lambda\!)\! \hat{V}_t \!
\!-\! \alpha_t \!  (\!\gamma \kappa(\!\bby_t,\! \cdot\!) \!
 - \!\kappa(\!\bbx_t,\!\cdot\!)\!)z_{t+1}\!\! \Big)\!\Big\rVert_{\ccalH}^2, \nonumber \\
&:=\!\ccalP_{\ccalH_{\bbD_{t+1}}} \!\!\Big[\! (1\! - \!\alpha_t \lambda) V_t\! -\! \alpha_t (\gamma \kappa(\bby_t, \cdot) \! -\! \kappa(\bbx_t,\cdot))z_{t+1} \Big] .
\end{align}%\vspace{-8mm}
%%
where we define the projection operator $\ccalP$ onto subspace $\ccalH_{\bbD_{t+1}}\subset \ccalH$ by the update \eqref{eq:projection_hat}. This orthogonal projection is the modification of the functional SQG iterate [cf. \eqref{eq:quasi_fsgd}] defined at the beginning of this subsection \eqref{eq:quasi_projected_fsgd}. Next we discuss how this update amounts to modifications of the parametric updates \eqref{eq:param_update} defined by functional SQG.
%
These subspace projections may be computed efficiently by exploiting the kernel parameterization described in Appendix \ref{apx_parameterization} operating together with destructive matching pursuit \cite{Vincent2002}.


%We proceed to describe the construction of these subspace projections. Consider subspaces $\ccalH_\bbD \subseteq \ccalH$ that consist of functions that can be represented using some dictionary $\bbD = [\bbd_1,\ \ldots,\ \bbd_M] \in \reals^{p \times M}$, i.e., $\ccalH_\bbD =\text{span}\{\kappa(\bbd_n, \cdot) \}_{n=1}^M$ . For convenience, we define $\boldsymbol{\kappa}_{\bbD}(\cdot)=[\kappa(\bbd_1,\cdot) \ldots \kappa(\bbd_M,\cdot)]$, and $\bbK_{\bbD,\bbD}$ as the resulting kernel matrix from this dictionary. We {enforce} function parsimony by selecting dictionaries $\bbD$ that $M_t << \ccalO(t)$.

%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% A  L  G  O  R  I  T  H  M  %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}[t]
\caption{PKGTD: Parsimonious Kernel Gradient Temporal Difference}
\begin{algorithmic}
\label{alg:pkgtd}
\REQUIRE $\{\bbx_t,\pi(\bbx_t), \bby_t,\alpha_t,\beta_t,\eps_t \}_{t=0,1,2,...}$
\STATE \textbf{initialize} ${V}_0(\cdot) = 0, \bbD_0 = [], \bbw_0 = [], z_0=0$, i.e. initial dict., coeffs., and aux. variable null
\FOR{$t=0,1,2,\ldots$}
	\STATE Obtain trajectory realization $(\bbx_t,\pi(\bbx_t), \bby_t)$
	\STATE Compute the TD and auxiliary sequence $z_{t+1}$  [cf. \eqref{eq:td_average}]:\vspace{-2mm}
%	
$$\quad \delta_t = r(\bbx_t, \pi(\bbx_t), \bby_t) + \gamma V_t(\bby_t) - V_t(\bbx_t),$$
$$z_{t+1} = (1-\beta_t) z_t + \beta_t \delta_t$$\vspace{-4.5mm}
%
	\STATE Compute unconstrained functional SQG step [cf. \eqref{eq:quasi_fsgd}]\vspace{-2mm}
	$$\tilde{V}_{t+1}(\cdot) =(1-\alpha_t \lambda)\tilde{V}_t(\cdot) - \alpha_t (\gamma \kappa(\bby_t, \cdot) - \kappa(\bbx_t,\cdot))z_{t+1}$$\vspace{-4.5mm}
	%
	\STATE Revise dict. $\tbD_{t+1} = [\bbD_t,\;\! \bbx_t \; , \bby_t ]$, weights $\tbw_{t+1} \leftarrow [(1-\alpha_t\lambda)\bbw_t,\;\;\alpha_t z_{t+1} ,-\alpha_t \gamma z_{t+1}]$%\vspace{-2mm}
	\STATE Compress dictionary via Alg. \ref{alg:komp}, obtain coeffs. via \eqref{eq:proximal_hilbert_representer} %\vspace{-2mm}
	$$({V}_{t+1},\bbD_{t+1},\bbw_{t+1}) = \textbf{KOMP}(\tilde{V}_{t+1},\tbD_{t+1},\tbw_{t+1},\epsilon_t)$$\vspace{-3mm}
\ENDFOR
\end{algorithmic}
\end{algorithm}



%This criterion amounts to finding the element $\tbd_\gamma$ of $\tbD$ which has maximal correlation (coherence) with the error residual (see \cite{Vincent2002}). Then, this dictionary element $\tbd_\gamma$ is added to the parsimonious dictionary $\bbD$. To obtain the resulting sparse function $f$, we compute its coefficient parameters $\bbw$ using the a least-squares projection of the form \eqref{eq:hatparam_update}, where the dictionary parameterizing ${f}$ now includes the new point $\tbd_\gamma$. The algorithm then terminates if the residual threshold condition $\lVert r \rVert_{\ccalH} \leq \eps_t $ is satisfied. Note that the procedure will, in the worst case, stop with $\hat{f} = \tilde{f}$, i.e., $\hbD = \tbD$ and $\hbw = \tbw$, meaning that the latest feature vector is added to the kernel dictionary such that the model order grows as $M_{t+1}=M_t + 1$.

We summarize the overall method, Parsimonious Kernel Gradient Temporal Difference (PKGTD) in Algorithm \ref{alg:pkgtd}: we execute the stochastic projection of the functional SQG iterates onto sparse subspaces $\ccalH_{\bbD_{t+1}}$ stated in \eqref{eq:projection_hat}. With initial function null $V_0=0$ (empty dictionary $\bbD_0=[]$ and coefficients $\bbw_0=[]$),%\footnote{The notation $[]$ is used to denote the empty matrix or vector respective size $p\times0$ or $0$.} 
%
at each step, given an i.i.d. sample $(\bbx_t, \pi(\bbx_t),\bby_t)$ and step-sizes $\alpha_t, \beta_t$, we compute the \emph{unconstrained} functional SQG iterate $\tilde{V}_{t+1}(\cdot) = (1-\alpha_t \lambda)\tilde{V}_t(\cdot) - \alpha_t (\gamma \kappa(\bby_t, \cdot) - \kappa(\bbx_t,\cdot))z_{t+1}$ parameterized by $\tbD_{t+1}$ and $\tbw_{t+1}$ as stated in \eqref{eq:param_tilde}, which are fed into KOMP (Algorithm \ref{alg:komp} in Appendix \ref{apx_parameterization}) with budget $\eps_t$, i.e., $(V_{t+1}, \bbD_{t+1}, \bbw_{t+1})= \text{KOMP}(\tilde{V}_{t+1},\tilde{\bbD}_{t+1}, \tilde{\bbw}_{t+1},\eps_t)$.%\vspace{-3mm}

{
\begin{remark}\label{remark_twotimescale}\normalfont
%
While two time-scale stochastic approximation originally appeared in the 1980s \cite{Korostelev,ermoliev1983stochastic} for compositional stochastic programming with asymptotic stability established, their role in RL, namely, to form the foundation of actor-critic algorithms \cite{borkar1997actor,konda2003onactor} was more recent. 

A separate but related line of research in RL identifies their use not in actor-critic (which is at its core a policy search method), but instead in order to solve Bellman equations (approximate dynamic programming), beginning with \cite{sutton2009convergent}. In \cite{sutton2009convergent} the authors hypothesize that one possible reason for instability of temporal difference learning under function approximation (as detailed in \cite{tsitsiklis1997analysis}), is that these are \emph{not gradient algorithms} but instead stochastic fixed point iterations. Thus, their stability interacts in a more intricate manner with the function parameterization. By reformulating Bellman equations as optimization problems, these problems are identified as possessing compositional structure, and thus are amenable to two time-scale algorithms, yielding \emph{gradient temporal difference} learning (GTD). The derivation of PKGTD is structurally aligned with GTD in that its derivation generalizes the derivation of GTD, rather than actor-critic, although two time-scale methods are at the core of both approaches. 
\end{remark}}


 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%S U B   S  E   C   T   I    O    N    %%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Coefficient Update induced by Sparse Subspace Projections}\label{subsec:apx_coefficient}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%S U B   S  E   C   T   I    O    N    %%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\subsection{Dictionary Selection via Greedy Compression}\label{subsec:apx_dictionary}





%

==> Convergence.tex <==
%!TEX root = root.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   S  E  C  T  I  O  N  %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Convergence Analysis}\label{sec:convergence}%\vspace{-5mm}
%
{We now analyze the stability and memory requirements of Algorithm \ref{alg:pkgtd} developed in Section \ref{sec:algorithm}. In stochastic fixed-point methods such as TD learning{,} the interplay between the Bellman operator contraction \cite{bertsekas1978stochastic} and expectations prevents the construction of supermartingales underlying stochastic descent stability \cite{Robbins1951}. {Attempts to overcome this challenge based on stochastic backward-differences require the state space to be completely explored in the limit \emph{per step} (intractable when $|\ccalX| = \infty$) \cite{tsitsiklis1994asynchronous}, or stipulate that data dependent matrices be non-singular \cite{sutton2009convergent}, respectively.} Thus these methods must be analyzed using ideas from dynamical systems \cite{borkar2000ode}. 
%
 In contrast, we establish that Algorithm \ref{alg:pkgtd} belongs to the family of descent algorithms, and hence its behavior can be connected to that of supermartingales \cite{wang2013incremental} -- to the best of our knowledge, this is the first time supermartingales have been used in analyzing stochastic methods for MDPs. This is also true of GTD \cite{sutton2009convergent}, although it is analyzed using ODEs \cite{borkar2000ode}. 
}

%
%We now analyze the stability and memory requirements of Algorithm \ref{alg:pkgtd} developed in Section \ref{sec:algorithm}. Our approach is fundamentally different from stochastic fixed point methods such as TD learning{,} which are not descent techniques, and thus exhibit delicate convergence. The interplay between the Bellman operator contraction \cite{bertsekas1978stochastic} and expectations prevents the construction of supermartingales underlying stochastic descent {stability \cite{Robbins1951}.} Attempts to mitigate this issue, such as those based on stochastic backward-differences \cite{kiefer1952stochastic} (\cite{tsitsiklis1994asynchronous,jaakkola1994convergence}) or Lyapunov approaches \cite{borkar2000ode}, e.g., \cite{sutton2009convergent}, require the state space to be completely explored in the limit \emph{per step} (intractable when $|\ccalX| = \infty$), or stipulate that data dependent matrices be non-singular, respectively. Thus, there is a long-standing question of how to {perform} policy evaluation in MDPs under conditions applicable to practitioners {while also} guaranteeing stability. We provide an answer by connecting RKHS-valued stochastic quasi-gradient methods (Algorithm \ref{alg:pkgtd}) with coupled supermartingale theory \cite{wang2013incremental}.

%{\bf Iterate Convergence} 
Under the assumptions stated next, it is possible to derive the fact that the auxiliary variable $z_t$ and value function estimate $V_t$ satisfy supermartingale-type relationships, but their behavior is intrinsically coupled. We generalize recently developed coupled supermartingale tools in \cite{wang2013incremental}, i.e., Lemma \ref{lemma:coupled_supermartingale} in Appendix \ref{apx_assumptions}, to RKHSs in order to establish the following almost sure convergence result when the step-sizes and compression budget are diminishing. More specifically, we require the following technical definitions and conditions.

\subsection{Technical Assumptions and Definitions}\label{apx_assumptions1}


In particular, for further reference, we define the functional stochastic quasi-gradient of the regularized objective as
%
\begin{align}\label{eq:quasi_sg}
&\hat{\nabla}_V J(V_t, z_{t+1}; \bbx_t, \pi(\bbx_t), \bby_t )=\nonumber\\
&\qquad\qquad\qquad (\gamma \kappa(\bby_t, \cdot) - \kappa(\bbx_t,\cdot))z_{t+1}  + \lambda V_t \; ,
\end{align}
%
and its sparse-subspace projected variant as
%
\begin{align}\label{eq:projected_quasi_sg}
&\tilde{\nabla}_V J(V_t, z_{t+1}; \bbx_t, \pi(\bbx_t), \bby_t ) \\
&= \!\frac{1}{\alpha_t} \Big( \!V_{t} \!-\!  \ccalP_{ \ccalH_{\bbD_{t+1}}} \Big[ V_t \!-\! \alpha_t \hat{\nabla}_V J(V_t, z_{t+1}; \bbx_t, \pi(\bbx_t), \bby_t )\!\Big]\!\Big)  \; ,\nonumber
\end{align}
Note that the update \eqref{eq:quasi_projected_fsgd}, using \eqref{eq:projected_quasi_sg}, may be rewritten as a stochastic projected quasi-gradient step rather than a stochastic quasi-gradient step followed by set projection, i.e.,
%
\begin{equation}\label{eq:quasi_projected_fsgd_projected}
V_{t+1} =V_t - \alpha_t \tilde{\nabla}_V J(V_t, z_{t+1}; \bbx_t, \pi(\bbx_t), \bby_t )  \; ,
\end{equation}
%

{Further, define the time-dependent sigma algebra, i.e., filtration, as  $\ccalF_t \supset (\{V_s, z_s,\bbx_s, \pi(\bbx_s), \bby_s\}_{s=0}^{t-1})$.} Now we are ready to state the technical conditions required for convergence. All statements involving conditional expectations are imposed with probability $1$, unless otherwise stated.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   A   S   S   U   M   P   T   I   O   N   %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%compact data domain
\begin{assumption}\label{as:first}
The state space $\ccalX\subset\reals^p$ and action space $\ccalA\subset \reals^q$ are compact, and the reproducing kernel map may be bounded as
%
\begin{equation}\label{eq:bounded_kernel}
\sup_{\bbx\in\ccalX} \sqrt{\kappa(\bbx, \bbx )} = X < \infty
\end{equation}
%
%Furthermore, the subspaces $\ccalH_{\bbD_{t}}$ output by Algorithm \ref{alg:komp} are intersected with some finite Hilbert-norm ball: $\|f\|_\ccalH \leq K$ for all $t$.
\end{assumption}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%  A  S  S  U  M  P  T  I  O  N  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
\begin{assumption}\label{as:mean_variance_td} % Define $\bar{\delta}_t = \mathbb{E}[\delta_t \given \bbx_0, \pi(\bbx_0)]$.
%%
The temporal difference $\delta$ and auxiliary sequence $z$ [cf. \eqref{eq:td_average}] satisfy the zero-mean and finite conditional variance conditions, respectively,
%%
\begin{align}\label{eq:td_assumption}
&\mathbb{E}\left[\delta \given \bbx, \pi(\bbx) \right] =\bar{\delta} \; ,
 \qquad\quad \mathbb{E}\left[(\delta - \bar{\delta})^2 \given \ccalF_t \right] \leq \sigma_{\delta}^2 \; , \nonumber\\
& \mathbb{E}\left[z^2 \given \bbx, \pi(\bbx) \right] \leq G_{\delta}^2\; .
\end{align}
%%
where  $\sigma_{\delta}$ and $G_{\delta}$ are positive scalars. 
%
\end{assumption}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%  A  S  S  U  M  P  T  I  O  N  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{assumption}\label{as:mean_variance_frechet} 
The stochastic quasi-gradient, when evaluated at $\bar{\delta}$, is an unbiased estimate for the true gradient $\nabla_V J(V)$. Moreover, the difference of reproducing kernels expression (the first factor in \eqref{eq:stoch_grad}) has finite conditional variance:
%
\begin{align}\label{eq:value_kernel_assumption}
%%
&\mathbb{E}\left[ (\gamma\kappa(\bby, \cdot) - \kappa(\bbx,\cdot)) \bar{\delta} \right] = \nabla_V J(V) \; , \nonumber\\
& \mathbb{E}\left[ \| \gamma\kappa(\bby_t, \cdot) - \kappa(\bbx_t,\cdot)\|_{\ccalH}^2 \given \ccalF_t \right ] \leq G_{V}^2 \; . 
\end{align}
%
Additionally, the projected stochastic gradient of the objective [cf. \eqref{eq:projected_quasi_sg}] has finite second conditional moment as
%
\begin{equation}\label{eq:projected_quasi_sg_variance}
\mathbb{E}\left[\|\tilde{\nabla}_V J(V_t, z_{t+1}; \bbx_t, \pi(\bbx_t), \bby_t ) \|_{\ccalH}^2 \given \ccalF_t \right] \leq \sigma_V^2 \; ,
\end{equation}
%
and the conditional mean of the temporal difference $\bar{\delta}$ is Lipschitz continuous with respect to the value function $V$, i.e for any two distinct $\delta$ and $\tilde{\delta}$, we have
%
\begin{align}\label{eq:td_lipschitz}
%%
|\bar{\delta} - \bar{\tilde{\delta}}  | \leq L_{V} \| V - \tilde{V} \|_{\ccalH}
%
\end{align}
%%
where $V,\tilde{V} \in \ccalH$ are distinct RKHS elements, $L_V >0$ is a scalar, and $ \bar{\delta} = \mathbb{E}_{\bby} [ r(\bbx, \pi(\bbx), \bby) + \gamma V(\bby) - V(\bbx) \given \bbx, \pi(\bbx)] $.
\end{assumption}

Assumption \ref{as:first} regarding the compactness of the state and action spaces of the Markov Decision Process intrinsically hold for most application settings and limit the radius of the set from which the MDP trajectory is sampled. Similar boundedness conditions on the reproducing kernel map have been considered in supervised learning applications \cite{Kivinen2004}. The mean and variance properties of the temporal difference stated in Assumption \ref{as:mean_variance_td} to bound the error in the descent direction associated with stochastic approximations, and are necessary to establish stability of stochastic methods. Assumption \ref{as:mean_variance_frechet} is similar to Assumption \ref{as:mean_variance_td} but instead of establishing bounds on the stochastic approximation error of the temporal difference, limits stochastic error variance in the reproducing kernel Hilbert space. These are natural extensions of the conditions needed for convergence of stochastic compositional gradient methods with vector-valued decision variables \cite{wang2017stochastic}. {However, we note that \eqref{eq:td_lipschitz}, in the context of MDPs, restricts the class of reward functions to be those which may be smoothly interpolated in a RKHS.} {This condition holds, for instance, when the reward is a potential or navigation-like function \cite{rimon1992exact,ngicml1999}, which are well-known to interact favorably in the design of controllers from a dynamical systems perspective.}

{The stipulation that the KOMP projection explicitly thresholds the norm of the value functions allows us to write}
\begin{equation}\label{eq:bounded_iterates}
\| V_t \|_{\ccalH} \leq K \; , \qquad \|V^* \|_{\ccalH} \leq K \; , \quad \text{ for all } t
\end{equation}
%
where $K>0$ is some constant. The boundedness of $V^*$ follows from the fact that since $\ccalX$ is compact and $J(V)$ is a continuous convex function over a compact set, its minimizer is achieved over this compact set \cite{brezis2010functional}[Corrolary 3.23].


%\vspace{-6mm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%  T  H  E  O  R  E  M   %%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{theorem}\label{theorem:convergence_wp1}
%
Consider the sequence $z_t$ [cf. \eqref{eq:td_average}] and $\{V_t\}$ [cf. \ref{eq:quasi_projected_fsgd}] as stated in Algorithm \ref{alg:pkgtd}. Assume the regularizer is positive $\lambda > 0$, Assumptions \ref{as:first} - \ref{as:mean_variance_frechet} hold, with the step-size conditions:
%
%
%
%\vspace{-2mm}
%
\begin{align}\label{eq:step_size_condition}
%
\!\!\!\sum_{t=1}^\infty\! \alpha_{t} \!=\!\infty \; ,\   \sum_{t=1}^\infty\! \beta_t \!= \!\infty , \  %\nonumber\\
\sum_{t=1}^\infty\! \alpha_{t}^2 \!+ \! \beta_t^2\!+\! \frac{\alpha_t^2}{\beta_t} \!\! <\!\! \infty\;, \ \eps_t \!= \!\alpha_t^2
%
\end{align}
%
Then $V_t \rightarrow V^*$ [cf. \eqref{eq:main_prob}] with probability $1$, and thus achieves the regularized Bellman fixed point \eqref{eq:bellman_operator_v_reformulate1} restricted to the RKHS.%\vspace{-1mm}
%
\end{theorem}%\vspace{-2mm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%  P  R  O  O  F  %%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{myproof} See Appendix \ref{apx_theorem_convergence_wp1}. \end{myproof}
%


The proof is given in Appendix \ref{apx_theorem_convergence_wp1}. Theorem \ref{theorem:convergence_wp1} states that the value functions generated by Algorithm \ref{alg:pkgtd} converge a.s. to the optimal $V^*$ defined by \eqref{eq:main_prob}. {With regularizer $\lambda$ made small but nonzero, using a universal kernel (e.g., a Gaussian), $V_t$ converges close to a function satisfying Bellman's equation in \emph{infinite MDPs} \eqref{eq:bellman_operator_v}. By decreasing the regularizer, limiting solutions close in on those which satisfy Bellman's  equation, though precise notions of closeness require continuity which is difficult to verify, given an arbitrary bounded reward. }This is the first guarantee w.p.1 for a true stochastic descent method with an infinitely and nonlinearly parameterized value function.  
%
Theorem  \ref{theorem:convergence_wp1} requires attenuating step-sizes such that the stochastic approximation error approaches null. In contrast, constant learning rates allow for maintaining algorithm adaptivity, motivating the following result.

One step-size sequence which satisfies the attenuation conditions \eqref{eq:step_size_condition} is 
%
%\begin{align}\label{eq:step_size_condition_example}
%%
%\alpha_t =\ccalO( t^{-(3/4 +\zeta/2)} )\; , \beta_t = \ccalO(t^{-(1 +\zeta)/2 })\; , \eps_t=\ccalO(\alpha_t^2) = \ccalO(t^{-(3/2 + \zeta)})
%%
%\end{align}
%
$\alpha_t =\ccalO( t^{-(3/4 +\zeta/2)} )\; , \beta_t = \ccalO(t^{-(1 +\zeta)/2 })\; , \eps_t=\ccalO(\alpha_t^2) = \ccalO(t^{-(3/2 + \zeta)})$, where $\zeta>0$ is an arbitrarily small constant so that series $\sum_t \alpha_t$ and $\sum_t \beta_t$ diverge. Generally, satisfying \eqref{eq:step_size_condition}, requires: $\alpha_t = \ccalO(t^{-p_{\alpha}})$, $\beta_t = \ccalO(t^{-p_{\beta}})$ with $p_{\alpha}\in(3/4, 1)$ and $p_{\beta}\in (1/2, 2 p_{\alpha}- 1)$.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%  T  H  E  O  R  E  M  %%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{theorem}\label{theorem:constant_stepsize_convergence}
%
Suppose Algorithm \ref{alg:pkgtd} is run with constant positive learning rates $\alpha_t=\alpha$ and $\beta_t=\beta$ and constant compression budget $\eps_t=\eps$ with sufficiently large regularization, i.e.%\vspace{-2mm}
%
\begin{align}\label{eq:constant_stepsize_parameters}
%
0<\beta < 1 \; , \alpha =\beta, \eps=C \alpha^2, \lambda=G_V^2 + \lambda_0 
\end{align}
%
where $C>0$ is a scalar, and $0<\lambda_0 < 1$. Then, under Assumptions \ref{as:first} - \ref{as:mean_variance_frechet}, the sub-optimality sequence $\|V_t - V^*\|_{\ccalH}^2$ converges in mean to a neighborhood:%\vspace{-2mm}
\begin{align}\label{eq:constant_stepsize_convergence}
%
\! \! \liminf_{t\rightarrow \infty} \E{\|V_{t}\! -\! V^*\|_{\ccalH}^2}={\ccalO\left(\alpha  \right)} \; .
%
\end{align}
\end{theorem}%\vspace{-3mm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%  P  R   O  O  F   %%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{myproof} See Appendix \ref{apx_theorem_constant_stepsize_convergence}. \end {myproof}
Theorem \ref{theorem:constant_stepsize_convergence} (proof in Appendix \ref{apx_theorem_constant_stepsize_convergence}) establishes that the value function estimates generated by Algorithm \ref{alg:pkgtd} converge in expectation to a neighborhood when constant step-sizes $\alpha$ and $\beta$ and sparsification budget $\epsilon$ in Algorithm \ref{alg:komp} are small constants. In particular, the bias $\eps$ induced by sparsification does not cause instability even when it is \emph{not going to null}. Moreover, this result only holds when the regularizer $\lambda$ is chosen large enough, which numerically induces a forgetting factor on past kernel dictionary weights \eqref{eq:param_tilde}. 
%
We may make the learning rates $\alpha$ and $\beta$ arbitrarily small, which yield a proportional decrease in the radius of convergence to a neighborhood of the Bellman fixed point \eqref{eq:bellman_operator_v}. 

{In general, Theorem \ref{theorem:constant_stepsize_convergence} \emph{does not} imply the sequence actually converges, but only that its $\liminf$ converges. To establish that the entire sequence converges, even in expectation, when used with constant step-sizes, one must recursively average the  functions and apply convexity of the objective function to establish the error bound decreases with the final iteration, as in Polyak-Ruppert averaging \cite{polyak1992acceleration}. Averaging, however, will be afflicted by the fact that different functions in the RKHS do not belong to the same subspace, and therefore their kernel dictionaries will need to be pooled, causing the model order to spike. Thus, averaging is a technique  of theoretical interest only in establishing limiting genuine behavior in RKHSs, and cannot be used unless parsimony is not a consideration. 
%
%Moreover, typically constant step-size analysis of stochastic methods requires a problem-dependent choice of step-size that depends on the strong convexity constant of the problem to ensure contraction across iterations -- again, see \cite{nemirovski2009robust}. Rather than approach the analysis in this manner, we instead treat the regularizer as tunable, as is conventional in learning methods.}
%
%Theorem \ref{theorem:constant_stepsize_convergence} is the first constant learning rate result for nonparametric compositional stochastic programming {of which we are aware}, and allows for repeatedly revising value function without the need for stochastic approximation error to approach null. 
%
By contrast, under constant step-sizes selection, the value function estimates have moderate complexity in the worst case.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% R  E  M  A  R  K  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{remark}\label{remark1} \normalfont
(Aggressive Constant Learning Rates)
In practice, one may obtain better performance by using larger constant step-sizes. To do so, the criterion \eqref{eq:constant_stepsize_parameters} may be relaxed: we require $0<\beta<1$ but $\alpha>0$ may be any positive scalar. Then, with regularizer chosen as $\lambda=G_V^2\frac{\alpha}{\beta} + \lambda_0 $ for $0<\lambda_0<1$, the radius of convergence is (see Appendix \ref{apx_theorem_constant_stepsize_convergence})%\vspace{-1mm}
%
\begin{align}\label{eq:constant_stepsize_convergence2}
&{\liminf_{t\rightarrow \infty} \E{\|V_{t} - V^*\|_{\ccalH}^2} }\nonumber\\
&\qquad =\ccalO\Big(\alpha^2 + \beta^2 + \frac{\alpha^2}{\beta}\Big[1 + \alpha^2 + \frac{\alpha}{\beta} + \frac{\alpha^2}{\beta^2}\Big] \Big) \; .
%
\end{align}
%
The ratios $\alpha^2/\beta$ and $\alpha^2/\beta^2$ dominate \eqref{eq:constant_stepsize_convergence2} and must be made small  to obtain accurate solutions. 
%
\end{remark}%\vspace{-2mm}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% R  E  M  A  R  K  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{remark}\label{remark2} \normalfont
(Regularization Path)
{In Theorem \ref{theorem:convergence_wp1}, we establish convergence for any $\lambda>0$ when step-sizes attenuate. That regularizer $\lambda$ may not be null means that we do not extract the exact Bellman fixed point restricted to the RKHS, but only a function that is close. In related work the minimizer $V_{\lambda}^*$ continuously depends on $\lambda$. It's beyond the scope of this work to extend these results to this setting, but on the hypothesis that they generalize to \eqref{eq:main_prob}, we may claim that decreasing $\lambda$ causes $V_{\lambda}^*$ to be closer to fixed point stated in \eqref{eq:bellman_operator_v}. 

On the other hand, for Theorem \ref{theorem:constant_stepsize_convergence} with given regularizer $\lambda$, imposes explicit restrictions on the choice of constant algorithm step-sizes. That is, we require $\lambda=G_V^2\frac{\alpha}{\beta} + \lambda_0 $ for $0<\lambda_0<1$, where $\alpha > 0$ and $0<\beta<1$. It is possible to derive the fact that larger regularization means faster learning rates but to less accurate solutions, in either diminishing or constant step-size settings, but these facts, which depend on rate analyses, are left to future work.}
\end{remark}\vspace{-3mm}
%


%{\bf Model Order Control}
As noted in Section \ref{sec:algorithm}, the complexity of functional stochastic quasi-gradient method in a RKHS is of order $\ccalO(2(t-1))$ which grows without bound. {To surmount this challenge, we propose subspace projections in Section \ref{subsec:polk_projection}.}  We {formalize here} that this projection indeed controls complexity when constant learning rates and compression budget are used. This result is a corollary, as it extends Theorem 3 in \cite{koppel2019parsimonious}. To obtain this result (proof in Appendix \ref{apx_corollary1}), we require the reward function to be bounded, as we state next.

%To establish Corollary \ref{corollary1}, we require the following condition.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%  A  S  S  U  M  P  T  I  O  N  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{assumption}\label{as:reward} 
The reward $r: \ccalX \times \ccalA \times \ccalX \rightarrow \reals$ is bounded:
%
\begin{equation}\label{eq:bounded_reward}
r(\bbx_t, \pi(\bbx_t), \bby_t) \leq R_{\max} \; \text{ for all } t, \bbx, \bba, \bby
%
\end{equation}
%
\end{assumption}

Assumption \ref{as:reward} holds whenever the reward function is continuous and the state and action spaces are compact, and thus holds for many popular RL problems. In this setting, the complexity of Algorithm \ref{alg:pkgtd} is finite, as is formalized next.

\begin{figure*}[t]
\centering
\vspace{-5mm}
%\hspace{-1mm}
 %\hspace{.85cm}
  \includegraphics[width=10cm,height=1cm]{figures/legend.pdf}\\
  %
 % \begin{subfigure}{\textwidth}
%\hspace{-9mm} 
\hspace{1mm} \includegraphics[width=5.75cm,height=5cm]{figures/error.pdf}\hspace{2mm}
%  \end{subfigure}
  %
  % \begin{subfigure}{\textwidth}
    \includegraphics[width=5.75cm,height=5cm]{figures/model.pdf}\hspace{2mm}
     % \end{subfigure}
      %
    %     \begin{subfigure}{\textwidth}
%    \vspace{-2mm}
  \includegraphics[width=5.8cm,height=5.1cm]{figures/value.pdf}%\hspace{-9mm}
     %   \end{subfigure}
%  \vspace{-2mm}  \includegraphics[width=.4cm,height=1cm,trim=0cm 0cm 17.5cm 22.65cm]{figures/value_legend2.pdf}%\hspace{-4cm}
  %\vspace{-2mm}
  \caption{Experimental comparison of PKGTD to existing kernel methods for policy evaluation on the Mountain Car task. Test set  error (left), and the parameterization complexity (center) vs. iterations. PKGTD learns fastest and most stably with the least complexity (best viewed in color). We plot the contour of the learned value function (right): its minimal value is in the valley, and states near the goal are close to null. Bold black dots are kernel dictionary elements, or retained instances. {Sample means and standard deviations of performance metrics (left and center) are generated via $100$ individual training runs.} }%{(i) is there any way we can display a contour plot of what the limiting value function looks like extracted by PKGTD which would yield a three-column figure? One benefit of nonparametric regression techniques is their interpretability. (ii) Also, to disambiguate the different algorithm sample paths, maybe half of them should be dotted. Basic colors like red, black, blue, green are easiest to distinguish on grey-scale.}}
  \label{fig:experiments}\vspace{-2mm}
\end{figure*}%\vspace{-3mm}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   C  O  R  R  O  L  A  R  Y   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{corollary}\label{corollary1}
%
Denote $V_t$ as the value function of Algorithm \ref{alg:pkgtd} with constant step-sizes $\alpha_t = \alpha$ and $\beta_t = \beta \in (0, 1)$ with compression budget $\eps_t =  \eps =C \alpha^2 $ and regularization $\lambda=(\alpha/\beta) G_V^2 + \lambda_0= \ccalO(\alpha\beta^{-1}+1) $  as in Remark \ref{remark1}. Let $M_t$ be its associated model order, i.e., the number of columns in its dictionary. Then there exists a finite upper bound $M^\infty$ such that, for all $t\geq0$, the model order is bounded $M_t\leq M^\infty$.%, and the limiting function $V^\infty=\lim_t V_t$ is finite.
%
\end{corollary}
%
%\vspace{1.5mm}

%
%\end{table*}
%\end{centering}
%
%{The result above, whose proof is given in Appendix \ref{apx_corollary1}, establishes} that Algorithm \ref{alg:pkgtd} yields convergent behavior for the problem \eqref{eq:main_prob} in both diminishing and constant step-size regimes. {With diminishing step-sizes [cf. \eqref{eq:step_size_condition}] and compression budget $\eps_t = \ccalO(\alpha_t^2)$, we obtain} exact convergence with probability $1$ of the function sequence $\{V_t\}$ in the RKHS to that of the regularized Bellman fixed point of the evaluation equation $V^*$ (Theorem \ref{theorem:convergence_wp1}). This result holds for any positive regularizer $\lambda>0$, and thus can be made arbitrarily close to the \emph{true Bellman fixed point} $V^{\pi}$ [cf. \eqref{eq:bellman_value}] by decreasing $\lambda$. {However, an exact solution requires} increasing the complexity of the function estimate such that its limiting memory becomes infinite.
%
%This drawback {motivates us to consider the case where} both the learning rates $\alpha_t = \alpha$, $\beta_t=\beta$ and the compression budget $\eps_t = \eps$ are constant. 
{Under specific selections \eqref{eq:constant_stepsize_parameters}, the {algorithm converges to a neighborhood} of the optimal {value function, whose radius depends} on the step-sizes, and may be made small by decreasing $\alpha$ at the cost of a decreasing learning rate. More importantly, {the use} of constant step-sizes and compression budget with large enough regularization yields a value function parameterized by a dictionary whose model order is always bounded (Corollary \ref{corollary1}). Thus, we may converge to an optimal neighborhood while ensuring the memory of the function parameterization is under control, and in the worst-case related to the covering number (metric entropy) of the state space.}%These results are summarized in Table \ref{tab2}. %\vspace{-3mm}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%  T  A  B  L  E    %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{table*}[]\centering\hfill
%\renewcommand{\arraystretch}{1.7}
%\caption{Summary of convergence results for different parameter selections.}
%\label{tab2}
%\begin{tabular}{llll}
%\cline{1-4}  
%$\qquad$ & $\!\!\! \! \! \!  $ Diminishing & $\!\!\! \! \! \! $ Constant &   $ \ $
%\\
%%
%\cline{1-4} 
%Learning rate      & $\!\! \! \! \! \sum_{t=1}^\infty \alpha_{t}^2 +  \beta_t^2+ \frac{\alpha_t^2}{\beta_t}  < \infty
%\; $       &   $ \!\! \! \! \!  \alpha > 0$, $\beta \in (0, 1)$   \\  
%Compression Budget       &$\!\! \! \! \!   \eps_t=\ccalO(\alpha_t^2 )$       &  $\!\! \! \! \!  \eps =\ccalO(\alpha^2) $     \\  
%Regularization       & $\!\! \! \! \!  0< \lambda $       &  $ \!\! \! \! \!  \lambda=\ccalO(\alpha\beta^{-1} + 1) $     \\  
%Convergence Result                & $\!\! \! \! \!  V_t \rightarrow V^*$ a.s.            & %
%$\!\! \! \! \! \sup \E{\|V_{t}\! -\! V^*\|_{\ccalH}^2} \rightarrow \ccalO\left(\alpha + \alpha^2 +\alpha^3 \right)$  \\ 
%Model Order               & $\!\! \! \! \! $ None            &  $\!\! \! \! \! $Finite  \\ 
%\cline{1-4}
%\end{tabular}%\vspace{-4mm}
%\end{table*}



==> Discussion.tex <==
%!TEX root = root.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   S  E  C  T  I  O  N    %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace{-3mm}
\section{Conclusion}\label{sec:discussion}%\vspace{-2.5mm}
%
In this paper, we considered the problem of policy evaluation in infinite MDPs with value functions that belong to a RKHS.  To solve this problem, we extended recent SQG methods for compositional stochastic programming to a RKHS, and used the result, combined with greedy sparse subspace projection, in a new policy-evaluation procedure called PKGTD (Algorithm \ref{alg:pkgtd}).  Under diminishing step sizes, PKGTD solves Bellman's evaluation equation exactly under the hypothesis that its fixed point belongs to a RKHS (Theorem \ref{theorem:convergence_wp1}).  Under constant step sizes, we can further guarantee finite-memory approximations (Corollary \ref{corollary1}) that still exhibit mean convergence to a neighborhood of the optimal value function (Theorem \ref{theorem:constant_stepsize_convergence}).  In our Mountain Car experiments, PKGTD yields excellent sample efficiency and model complexity, and therefore holds promise for large state space problems common in robotics where fixed state-action space tiling may prove impractical.

\vspace{-2mm}

==> Experiments.tex <==
%!TEX root = root.tex
\vspace{-2mm}
\section{Experiments}
\label{sec:experiments}
%\vspace{-.5cm}
%
%
%\begin{figure*}
%
%\setcounter{subfigure}{0}
%\hspace{-2mm}\begin{subfigure}{.7\columnwidth}
%\includegraphics[width=\linewidth, height = 0.8\linewidth]
%                {figures/error.pdf}
%\caption{Relative error vs. iteration $t$}
%\label{subfig:field_snapshot}
%\end{subfigure}\hspace{-3mm}
%
%\begin{subfigure}{.75\columnwidth}
%\includegraphics[width=\linewidth,height = 0.7\linewidth]
%                {figures/model.pdf}
%\caption{Model complexity vs. iteration $t$}
%\label{subfig:objective}
%\end{subfigure}\hspace{-4mm}
%
%\begin{subfigure}{.75\columnwidth}
%\includegraphics[width=\linewidth,height = 0.7\linewidth]
%                {figures/value2.pdf}
%                \includegraphics[width=1.25cm,height=2.25cm]{figures/value_legend2.pdf}
%\caption{Value of states}
%\includegraphics[width=1.25cm,height=2.25cm]{figures/value_legend2.pdf}
%\label{subfig:proximity}
%\end{subfigure}
%
%\caption{Experimental comparison of PKGTD to existing kernel methods for policy evaluation on the Mountain Car task. Test set  error \eqref{eq:test_error} (left), and the parameterization complexity (center) vs. iterations. PKGTD learns fastest and most stably with the least complexity (best viewed in color). On the right, we plot a contour plot of the learned value function: observe that its minimal value is in the valley, and states near the goal are close to null. Bold black dots are kernel dictionary elements..}\label{fig:fields}%\vspace{-3mm}
%\end{figure*}
%


Our experiments aim to compare PKGTD to other policy evaluation techniques in this domain.  Because it seeks memory-efficient solutions over an RKHS, we expect PKGTD to obtain accurate estimates of the value function using only a fraction of the memory required by the other methods.
%
We perform experiments on the classical Mountain Car domain \cite{sutton1998reinforcement}: an agent applies discrete actions $\ccalA = \left\{ \texttt{reverse}, \texttt{coast}, \texttt{forward} \right\}$ to a car that starts at the bottom of a valley and attempts to climb up to a goal at the top of one of the mountain sides. The state space is continuous, consisting of the car's scalar position and velocity, i.e., {$\ccalX \subset \reals^2$}.  The reward function $r(\bbx_t,\bba_t,\bby_t)$ is $-1$ unless $\bby_t$ is the goal state at the mountain top, in which case it is $0$ and the episode terminates.



Now we describe the configuration of the algorithms used for comparison. The Mountain Car environment has a two-dimensional state space (position and velocity) with bounds of $[-1.2, 0.6]$ in position, and $[-0.07, 0.07]$ in velocity. We chose not to normalize this state space to $[0,1]$ intervals, choosing instead to handle the scale difference by using non-isotropic kernels. The ratio of the kernel variances is equal to the ratio of the lengths of their corresponding bounds, so they would be isotropic kernels if we normalized the state space.

We used a fixed non-isotropic kernel bandwidth of $\sigma_1 = 0.2, \sigma_2 = 0.0156$ in all cases. By fixing the kernel bandwidth across all algorithms, we are basically enforcing that the learned functions all belong to the same Kernel Hilbert Space.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   PARAMETERS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%\section{Experimental Details}\label{sec:parameters}
%\vspace{-3mm}\begin{centering}
%\begin{table*}\centering\hfill
%\renewcommand{\arraystretch}{1.7}
%\caption{Experiment Parameters}
%\label{tab:parameters}
%\vspace{3mm}


For PKGTD, the relevant parameters are the step size, $\alpha$, the rate of expectation update, $\beta$, the regularizer, $\lambda$, and the approximation error, $K$. For GPTD, the relevant parameters are the gaussian process noise standard deviation, $\sigma_0$, the linear independence test bound, $\nu$, and the regularizer, $\lambda$. For the RBF grids fit using GTD, the relevant parameters are the grid spacing in the position and velocity directions, $h_1$ and $h_2$, respectively, the step size, $\alpha$, and the rate of expectation update, $\beta$. Our values are summarized in Table 1. {While theoretically the selection of $\lambda$ is sensitive, experimentally we find it to have little impact, and thus fix it as a small value $\lambda = 10^{-6}$. 
%\vspace{2mm}
\begin{tabular}{lcccccccc}
           &   \hspace{-2mm} $\alpha$ &\hspace{-6mm} $\beta$ & \hspace{-6mm} $\lambda$ & \hspace{-2mm} $K$   &  \hspace{-2mm} $\sigma_0$ &\hspace{-2mm} $\nu$ &\hspace{-2mm} $h_1$ & \hspace{-2mm}$h_2$  \\
  \cline{2-9}
  \hspace{-3mm} PKGTD    &  \hspace{-4mm} 8.0      & \hspace{-4mm}0.2     &  \hspace{-2mm}1e-6      &  \hspace{-2mm}0.02  &    \hspace{-2mm}        &       &       &        \\
\hspace{-3mm}  GPTD     &     \hspace{-4mm}      &     \hspace{-4mm}    &  \hspace{-2mm}1e-6      &     \hspace{-2mm}   &\hspace{-2mm} 0.01       & 0.2   &       &        \\
\hspace{-3mm}  RBF-25   & \hspace{-4mm} 10.0     &\hspace{-4mm} 0.25    &     \hspace{-2mm}       &    \hspace{-2mm}    &  \hspace{-2mm}          & \hspace{-2mm}      &\hspace{-2mm} 0.44  &\hspace{-2mm} 0.0343 \\
\hspace{-3mm}  RBF-49   & \hspace{-5.5mm} 1.5      & \hspace{-3mm}0.35    &       \hspace{-2mm}     &    \hspace{-2mm}    &    \hspace{-2mm}        &    \hspace{-2mm}   & \hspace{-1mm}0.26  & \hspace{-1mm}0.0203 \\
\end{tabular}\vspace{-1mm}
\begin{center}Table 1: Experimental Parameters\end{center}
%
%
Theoretically and experimentally, we require that $\beta \in (0,1)$. Selection of $\beta\approx 1/4$ was done by consulting values considered in the original GTD experiments, and $\alpha = 8$ or $\alpha=10$ was based on the fact that larger step-sizes yield faster learning, so it is advantageous to use step-sizes $\alpha$ an order of magnitude larger than $\beta$.}


To obtain a benchmark policy for this task, we make use of trust region policy optimization \cite{schulman2015trust}. To evaluate value function estimates, we form an offline training set of state transitions and associated rewards by running this policy through consecutive episodes until we had one training trajectory of 5000 steps and then repeat this for 100 training trajectories to generate sample statistics. For ground truth, we generate one long trajectory of 10000 steps and randomly sample 2000 states from it. From each of these 2000 states, we apply the policy until episode termination and use the observed discounted return as  $\hat{V}_\pi(\bbx)$. Since our policy was deterministic, we only performed this procedure once per sampled state. For value function $V$, we define the percentage error metric:
%
%\begin{equation}
$  \text{Percentage Error}(V) = ({1}/{2000}) \sum_{i=1}^{2000} | ({ V(\bbx_i) - \hat{V}_\pi(\bbx_i) })/{\hat{V}_\pi(\bbx_i) } |$
 % \label{eq:test_error}
%\end{equation}
%

We compared PKGTD with a Gaussian kernel to two other techniques for policy evaluation that also use kernel-based value function representations: (1) Gaussian process temporal difference (GPTD) \cite{engel2003bayes}, and (2) gradient temporal difference (GTD) \cite{sutton2009convergent} using radial basis function (RBF) network features.  We fix a kernel bandwidth across all techniques, and select parameter values that yield the best results for each method (see Table 1).  For RBF feature generation, we use two fixed grids with different spacing.  The first was one for which GTD yielded a value function estimate with percentage error similar to that which we obtained using PKGTD (RBF-49), and the second was one which yielded a number of basis functions that was similar to what PKGTD selected (RBF-25). 

{Figure~\ref{fig:experiments} displays these results: on the left we show percentage error, a surrogate for Bellman evaluation error, versus training example, in which we observe that PKGTD yields fast and reliable learning. In the center figure, we show the number of points in the kernel dictionary (model size) over samples, which demonstrates that PKGTD only keeps past states needed to estimate the value function well, rather than statistically insignificant points. %On the right, we display a contour plot of the limiting value function learned by PKGTD, which is readily interpretable.
%
Overall, we note that GTD with fixed RBF features requires a much denser grid in order to reach the same Percentage Error as Algorithm \ref{alg:pkgtd}, and that adaptive instance selection results in both faster initial learning and smaller error.  Compared to GPTD, which chooses model points online according to a fixed linear-dependence criterion, PKGTD requires fewer model points and converges to a better estimate of the value function more quickly and stably.

Fig. 1 (right) displays a contour plot of the value function -- the x-axis denotes position, the y-axis denotes velocity, and bold black dots denote kernel dictionary elements, i.e., past visited states that are essential for representing the estimate of $V^\pi$. The contour plot suggests that low value states are when one has small velocity near position $-0.6$ (the bottom of the hill). Moreover, value progressively increases as speed increases away from the bottom of the hill towards the top. 

 }

==> Experiments2.tex <==
%!TEX root = root.tex
\section{Experiments}
\label{sec:experiments}
\vspace{-.5cm}
 \hspace{.85cm} \includegraphics[width=8cm,height=.8cm]{figures/legend.pdf}
\begin{figure}[htpb]
\vspace{-5mm}
\hspace{-1mm}
  %
 % \begin{subfigure}{\textwidth}
  \includegraphics[width=4.7cm,height=3.7cm]{figures/error.pdf}\hspace{-1.5mm}
%  \end{subfigure}
  %
  % \begin{subfigure}{\textwidth}
    \includegraphics[width=4.7cm,height=3.7cm]{figures/model.pdf}\hspace{-1.5mm}
     % \end{subfigure}
      %
    %     \begin{subfigure}{\textwidth}
  \includegraphics[width=4.4cm,height=3.7cm]{figures/value2.pdf}\hspace{-9mm}
     %   \end{subfigure}
  \vspace{-2mm}  \includegraphics[width=.4cm,height=1cm,trim=0cm 0cm 16cm 20.65cm]{figures/value_legend2.pdf}%\hspace{-4cm}
  %\vspace{-2mm}
  \caption{Experimental comparison of PKGTD to existing kernel methods for policy evaluation on the Mountain Car task. Test set  error (left), and the parameterization complexity (center) vs. iterations. PKGTD learns fastest and most stably with the least complexity (best viewed in color). We plot the contour of the learned value function (right): its minimal value is in the valley, and states near the goal are close to null. Bold black dots are kernel dictionary elements, or retained instances. }%\blue{(i) is there any way we can display a contour plot of what the limiting value function looks like extracted by PKGTD which would yield a three-column figure? One benefit of nonparametric regression techniques is their interpretability. (ii) Also, to disambiguate the different algorithm sample paths, maybe half of them should be dotted. Basic colors like red, black, blue, green are easiest to distinguish on grey-scale.}}
  \label{fig:experiments}
\end{figure}\vspace{-3mm}

%
%
%\begin{figure*}
%
%\setcounter{subfigure}{0}
%\hspace{-2mm}\begin{subfigure}{.7\columnwidth}
%\includegraphics[width=\linewidth, height = 0.8\linewidth]
%                {figures/error.pdf}
%\caption{Relative error vs. iteration $t$}
%\label{subfig:field_snapshot}
%\end{subfigure}\hspace{-3mm}
%
%\begin{subfigure}{.75\columnwidth}
%\includegraphics[width=\linewidth,height = 0.7\linewidth]
%                {figures/model.pdf}
%\caption{Model complexity vs. iteration $t$}
%\label{subfig:objective}
%\end{subfigure}\hspace{-4mm}
%
%\begin{subfigure}{.75\columnwidth}
%\includegraphics[width=\linewidth,height = 0.7\linewidth]
%                {figures/value2.pdf}
%                \includegraphics[width=1.25cm,height=2.25cm]{figures/value_legend2.pdf}
%\caption{Value of states}
%\includegraphics[width=1.25cm,height=2.25cm]{figures/value_legend2.pdf}
%\label{subfig:proximity}
%\end{subfigure}
%
%\caption{Experimental comparison of PKGTD to existing kernel methods for policy evaluation on the Mountain Car task. Test set  error \eqref{eq:test_error} (left), and the parameterization complexity (center) vs. iterations. PKGTD learns fastest and most stably with the least complexity (best viewed in color). On the right, we plot a contour plot of the learned value function: observe that its minimal value is in the valley, and states near the goal are close to null. Bold black dots are kernel dictionary elements..}\label{fig:fields}%\vspace{-3mm}
%\end{figure*}
%


Our experiments aim to compare PKGTD to other policy evaluation techniques in this domain.  Because it seeks memory-efficient solutions over an RKHS, we expect PKGTD to obtain accurate estimates of the value function using only a fraction of the memory required by the other methods.
%
We perform experiments on the classical Mountain Car domain \cite{sutton1998reinforcement}: an agent applies discrete actions $\ccalA = \left\{ \texttt{reverse}, \texttt{coast}, \texttt{forward} \right\}$ to a car that starts at the bottom of a valley and attempts to climb up to a goal at the top of one of the mountain sides. The state space is continuous, consisting of the car's scalar position and velocity, i.e., $\ccalX = \reals^2$.  The reward function $r(\bbx_t,\bba_t,\bby_t)$ is $-1$ unless $\bby_t$ is the goal state at the mountain top, in which case it is $0$ and the episode terminates.

To obtain a benchmark policy for this task, we make use of trust region policy optimization \cite{schulman2015trust}. To evaluate a value function estimate, we form an offline training set of state transitions and associated rewards by running this policy through consecutive episodes until we had one training trajectory of 5000 steps and then repeat this for 100 training trajectories to generate sample statistics. For ground truth, we generate one long trajectory of 10000 steps and randomly sample 2000 states from it. From each of these 2000 states, we apply the policy until episode termination and use the observed discounted return as  $\hat{V}_\pi(\bbx)$. Since our policy was deterministic, we only performed this procedure once per sampled state. For value function $V$, we define the percentage error metric:
%
%\begin{equation}
$  \text{Percentage Error}(V) = ({1}/{2000}) \sum_{i=1}^{2000} | ({ V(\bbx_i) - \hat{V}_\pi(\bbx_i) })/{\hat{V}_\pi(\bbx_i) } |$
 % \label{eq:test_error}
%\end{equation}
%
We compared PKGTD with a Gaussian kernel to two other techniques for policy evaluation that also use kernel-based value function representations: (1) Gaussian process temporal difference (GPTD) \cite{engel2003bayes}, and (2) gradient temporal difference (GTD) \cite{sutton2009convergent} using radial basis function (RBF) network features.  None of the methods had access to prior knowledge about the optimal value function.

Figure~\ref{fig:experiments} depicts the results of our experiment. We fix a kernel bandwidth across all techniques, and select parameter values that yield the best results for each method (Appendix \ref{sec:parameters}).  For RBF feature generation, we use two fixed grids with different spacing.  The first was one for which GTD yielded a value function estimate with percentage error similar to that which we obtained using PKGTD (RBF-49), and the second was one which yielded a number of basis functions that was similar to what PKGTD selected (RBF-25). Observe that GTD with fixed RBF features requires a much denser grid in order to reach the same Percentage Error as Algorithm \ref{alg:pkgtd}.  Moreover, PKGTD's adaptive instance selection results in both faster initial learning and smaller  error.  Compared to GPTD, which chooses model points online according to a fixed linear-dependence criterion, PKGTD requires fewer model points and converges to a better estimate of the value function more quickly and stably. 

==> Introduction.tex <==
%!TEX root = root.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   S  E  C  T  I  O  N    %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\vspace{-16mm}
\vspace{-4mm}
\section{Markov Decision Processes}\label{sec:mdps}%\vspace{-1mm}
%
We consider an autonomous agent acting in an environment defined by a Markov decision process (MDP) \cite{sutton1998reinforcement} with continuous spaces, which is increasingly relevant to emerging technologies such as robotics \cite{kober2013reinforcement}, power systems \cite{scott2014least}, and others. A MDP is a quintuple $(\ccalX, \ccalA, \mathbb{P}, r, \gamma)$, where $\mathbb{P}$ is the action-dependent transition probability of the process: when the agent starts in state $\bbx_t \in \ccalX \subset \reals^p$ at time $t$ and takes an action $\bba_t \in \ccalA$, a transition to next state $\bby_t\in \ccalX$ is distributed according to 
%
%\begin{equation}\label{eq:transition_prob}
$\bby_t \sim \mathbb{P}(\cdot \given \bbx_t, \bba_t).$
%\end{equation}
%
After transitioning to a particular $\bby_t$, the MDP reveals an instantaneous reward $r(\bbx_t, \bba_t, \bby_t)$, where the reward function is a map $r :\ccalX \times \ccalA \times \ccalX \rightarrow \reals$. %\vspace{-.5mm}

 
We focus on \emph{policy evaluation}: control decisions $\bba_t$ are chosen according to a fixed stationary stochastic policy $\pi: \ccalX \rightarrow \rho(\ccalA)$, where $\rho(\ccalA)$ denotes the set of probability distributions over $\ccalA$. Policy evaluation underlies methods that seek optimal policies through repeated evaluation and improvement. In policy evaluation, we seek to compute the \emph{value} of a policy when starting in state $\bbx$, quantified by the discounted expected sum of rewards, or value function $V^{\pi}(\bbx)$:%\vspace{1.41mm}
 %
 \footnote{In MDPs more generally, we choose actions $\{\bba_t \}_{t=1}^\infty$ to maximize the reward accumulation  starting from state $\bbx$, i.e.,
%\begin{equation}\label{eq:value_function}
$V(  \bbx, \{\bba_t\}_{t=0}^\infty ) = \mathbb{E}_{\bby}\Big[\sum_{t=0}^\infty \gamma^t r(\bbx_t, \bba_t, \bby_t ) \given \bbx_0 = \bbx, \{\bba_t \}_{t=0}^\infty \Big].$ For a fixed policy $\pi$, the setting of this work, this simplifies to \eqref{eq:value_function}.}\vspace{2mm}
%\end{equation}
  %
\begin{align}\label{eq:value_function}
\!\!\!V^{\pi}\!(  \bbx ) \!=\! \mathbb{E}_{\bby}\!\Big[\!\sum_{t=0}^\infty \! \!\gamma^t  r(\bbx_t, \bba_t, \bby_t \!)  \!\given \! \bbx_0 \!=\! \bbx, \!\{\!\bba_t \!=\! \pi(\bbx_t)\!\}_{t=0}^\infty \! \Big].
\end{align}
%
%
For a single trajectory through the state space $\ccalX$, $\bby_t = \bbx_{t+1}$. The value function \eqref{eq:value_function} is parameterized by a discount factor $\gamma \in (0,1)$ that determines farsightedness. 
%
% When following policy $\pi$, we parameterize the value function \eqref{eq:value_function} by $\pi$, i.e., $V^{\pi}(\bbx)=\mathbb{E}[V(  \bbx, \{\bba_t \}_{t=0}^\infty ) \given \{ \bba_t = \pi(\bbx_t)\}_{t=0}^\infty ]$.
%
Decomposing the summand in \eqref{eq:value_function} into its first and subsequent terms, and using both the stationarity of the transition probability and the Markov property % [cf. \eqref{eq:transition_prob}]
yields the Bellman evaluation equation \cite{Bellman:1957}:%\vspace{-1mm}
  %
\begin{equation}\label{eq:bellman_value}
V^\pi( \bbx) = \int_{\ccalX} [ r(\bbx,\pi(\bbx),\bby) + \gamma V^{\pi}(\bby)] \mathbb{P}(d\bby \given \bbx, \pi(\bbx))
\end{equation}
%%
for all $\bbx \in \ccalX$.
The right-hand side of \eqref{eq:bellman_value} defines a Bellman evaluation operator $\bellman^\pi : \ccalB(\ccalX) \rightarrow \ccalB(\ccalX )$ over $\ccalB(\ccalX )$, the space of bounded continuous value functions $V:\ccalX\rightarrow \reals$:%\vspace{-3mm}
%
%\footnote{$\ccalB(\ccalX)$ is used to denote the space of real-valued bounded continuous functions defined over state space $\ccalX$.}
%
\begin{align}\label{eq:bellman_operator_v}
\!\!\!(\!\bellman^{\pi} V) (\bbx) \! =\!\!    \int_{\ccalX} \!\![ r(\bbx,\pi(\bbx) ,\bby)\! +\! \gamma V^{}(\bby)] \mathbb{P}(d\bby \given \bbx, \pi(\bbx) )
\end{align}
%%
for all $\bbx \in \ccalX$. {Proposition 4.2(b) in \cite{bertsekas1978stochastic}} establishes that the stationary point of \eqref{eq:bellman_operator_v} is $V^{\pi}$, i.e., $( \bellman^{\pi} V^\pi )(\bbx) = V^{\pi}(\bbx)$.
%
{As a stepping stone to finding optimal policies in infinite MDPs, we seek here to find the fixed point of \eqref{eq:bellman_operator_v}.  Specifically, the goal of this work is stable value function estimation in infinite MDPs, with nonlinear parameterizations that are allowed to be infinite, but are nonetheless memory-efficient.} %the Bellman evaluation operator when following a fixed policy $\pi$, a necessary precursor to finding the optimal policy.

%\vspace{-3mm}
%\subsection{}\label{sec:review}%\vspace{-2mm}
%

%discuss:
%computation of conditional expectation impossible in large MDPs --> stochastic approximation
{\bf Challenges } To solve \eqref{eq:bellman_operator_v}, fixed point methods, i.e., value iteration ($V_{k+1} = \bellman^{\pi} V_k$), have been proposed \cite{bertsekas1978stochastic}, but {can only be implemented in a memory-affordable manner} when the {value function can be represented by a vector whose length is defined by the number of states and the state space is small enough that the expectation\footnote{\noindent Observe that the integral in \eqref{eq:bellman_value} defines a conditional expectation: $V^\pi( \bbx) = \mathbb{E}_{\bby}[ r(\bbx,\pi(\bbx),\bby) + \gamma V^\pi(\bby)]  \given \bbx, \pi(\bbx)]$.} in $\bellman$ can be computed.} For large spaces, stochastic approximations of value iteration, i.e., temporal difference (TD) learning \cite{sutton1988learning}, circumvent computing expectations. 
%
Incremental methods (least-squares TD) are an alternative when $V(\bbx)$ is vector-valued \cite{bradtke1996linear}, but extensions to infinite representations require infinite memory \cite{powell2011review}. %or elude stability \cite{xu2005kernel}. 






Solving the fixed point problem defined by \eqref{eq:bellman_operator_v} requires surmounting the fact that this expression is defined for {each $\bbx \in \ccalX$}, which for continuous $\ccalX\subset \reals^p$ has \emph{infinitely many} unknowns. This phenomenon is one example of Bellman's curse of dimensionality \cite{Bellman:1957}, and it is frequently sidestepped by parameterizing the value function {using} a finite linear \cite{tsitsiklis1997analysis,melo2008analysis} or nonlinear \cite{bhatnagar2009convergent} basis expansion. Such methods {have} paved the way for the recent success of neural networks in value function-based approaches to MDPs{, but combining TD learning with different parameterizations may cause divergence \cite{Baird95residualalgorithms}: in} general, the representation must be tied to the stochastic update  \cite{jong2007model} to ensure both are stable.
%\vspace{-2mm}
%\subsection{Contributions}\label{subsec:contributions}%\vspace{-2mm}

{\bf Contributions } Our main result is a memory-efficient, non-parametric{,} stochastic method that converges to the Bellman fixed point almost surely when it belongs to a reproducing kernel Hilbert space (RKHS). The hypothesis that the value function belongs to a RKHS restricts the relationship between rewards and value to be smooth (see Assumption \ref{as:mean_variance_frechet} [cf. \eqref{eq:td_lipschitz}] ), i.e., large changes in rewards yield large changes in value., {which holds, for instance, when the reward is a potential or navigation function \cite{rimon1992exact,ngicml1999}. Such specifications are known to interact favorably in controller design from a dynamical systems perspective.} We reformulate \eqref{eq:bellman_value} as a compositional stochastic program (Section \ref{subsec:opt}), a topic studied in operations research \cite{shapiro2014lectures} and probability \cite{Korostelev}. These problems motivate stochastic \emph{quasi-gradient} (SQG) methods, i.e.,  two time-scale approaches, to mitigate the fact that the objective's stochastic gradient requires evaluating an expectation \cite{ermoliev1983stochastic}. 

{Two time-scale stochastic methods have a significant history in reinforcement learning in the context of a class of policy learning algorithms called actor-critic \cite{borkar1997actor}, which mix together gradient ascent on the value function \cite{sutton2000policy} with value function estimation through temporal differences \cite{sutton1988learning}. Alternatively, their utility also has been established for policy evaluation in \cite{bhatnagar2009convergent,sutton2009convergent} for finite MDPs or value functions that have finite vector-valued parameterizations. Our work is more closely related to this later context; however, a key point of departure is that we propose to operate directly in a function space, motivated by the fact that policy evaluation in a continuous MDP defines a functional fixed point problem.} Specifically, we use SQG in infinite MDPs. 

In \eqref{eq:bellman_value}, the decision variable is a continuous function, which we address by hypothesizing the Bellman fixed point belongs to a RKHS \cite{kimeldorf1971some}. However, a function in a RKHS has comparable complexity to the {number of training samples processed}, which could be infinite ({an issue} ignored in many kernel methods for MDPs \cite{ormoneit2002kernel,taylor2009kernelized,grunewalder2012modelling,JMLR:v17:13-016,dai2016learning}). {Specifically, it's well known that for a kernelized interpolator defined by a training set of $N$ samples, the complexity is $\ccalO(N)$. Thus, to solve the population problem defined by Bellman's equations, $N\rightarrow \infty$, and thus so is the complexity of the function estimate. We propose to tackle this memory bottleneck by requiring memory efficiency in both the function sample path and in its limit, whose complexity in the worst case is defined by the metric entropy of the state space (Corollary \ref{corollary1}).}

To find a memory-efficient sample path in the function space, we generalize {SQG to RKHSs} (Section \ref{sec:algorithm}), and combine {this generalization} with {greedily-constructed} sparse subspace projections (Section \ref{subsec:polk_projection}). {These subspaces are constructed via matching pursuit \cite{Pati1993,lever2016compressed}, {a procedure} motivated by the {facts} that kernel matrices induced by arbitrary data streams likely violate requirements for convex-relaxation-based sparsity \cite{candes2008restricted}. 
 %
Rather than unsupervised forgetting \cite{engel2003bayes}, we tie the projection-induced error to ensure the stochastic gradient still satisfies a descent property \cite{koppel2019parsimonious}, thus keeping only those dictionary points needed to converge (Section \ref{sec:convergence}). 

{Whereas in \cite{koppel2019parsimonious}, compressed kernel methods are analyzed for supervised learning and a tunable tradeoff between memory and sub-optimality is provided, here we study compressed kernel methods in the context of policy evaluation in reinforcement learning. This later context requires surmounting the technical challenges associated with nested expectations, specifically, that SQG is defined by coupled supermartingales, rather than standard stochastic descent arguments in \cite{koppel2019parsimonious}, and hence has fundamental qualitative and quantitative departures from existing works on RKHS learning.}

We note that this hard-thresholding projection could be applied to other stochastic algorithms in RKHS for reinforcement learning such as \cite{ormoneit2002kernel,taylor2009kernelized,grunewalder2012modelling,dai2016learning}, but applying them to incremental methods (LSTD) \cite{powell2011review,JMLR:v17:13-016} remains elusive since relating the per-step bias caused by sparsification to ensure valid descent directions is elusive.}

 
{As a result,} we conduct functional SQG descent via sparse projections of the SQG{. This maintains a moderate-complexity} sample path exactly towards $V^*$, which may be made arbitrarily close to {the Bellman fixed point} by decreasing the regularizer.
%
By generalizing the relationship between SQG and supermartingales in \cite{wang2017stochastic} to Hilbert spaces, we establish that the sparse projected SQG sequence converges almost surely to the Bellman fixed point with decreasing learning rates, and converges in mean while maintaining finite complexity when constant learning rates are used (Section \ref{sec:convergence}). We then empirically evaluate the proposed value function approximation method on the discrete Mountain Car domain in Section \ref{sec:experiments} and summarize our findings in Section \ref{sec:discussion}.% This is the first almost sure convergence result for policy evaluation in infinite MDPs with \emph{nonlinear value function parameterizations} of moderate complexity.%, which is in the worst-case comparable to the data domain covering number \cite{zhou2002covering,pontil2003note}. 
%

{
We would like to point out that convergence of two time-scale methods is well-understood \cite{wang2016accelerating,wang2017stochastic}; however, applying these methods as is requires decision variables to be \emph{vectors}, not \emph{functions}. This parameterization, however, causes an approximation error which is difficult to characterize (see \cite{JMLR:v17:13-016}). In contrast, the RKHS parameterization, operating with the combination of projections and SQG, attains solutions that are close to the minimizer of the true Bellman evaluation error, where closeness is controlled by regularization introduced in the next section. This is due to the fact that RKHS possesses universal approximation under judicious choice of the kernel \cite{micchelli2006universal}, thus circumventing approximation error.}
 %{ discussion of experiments goes here, says things work better than comparators}

{Recently, in companion work, an optimization-based variant of $Q$ learning in RKHS is developed \cite{tolstaya2018nonparametric}; however, a number of essential points distinguish that thread from methods developed here. Specifically, the optimization-based reformulation of Bellman's evaluation equation yields a convex program for which i.i.d. assumptions are close-to-valid. By contrast, Bellman's optimality equation yields a \emph{non-convex reformulation}. While the convergence of $Q$ learning requires i.i.d. assumptions, typically in practice these are violated. These statistical dependencies make policy learning a challenging domain to study Bayesian exploration, whereas policy evaluation is suitable \cite{precup2000eligibility}. Additionally, policy evaluation is just one component of reinforcement learning algorithms based upon policy search such as policy gradient method \cite{sutton2000policy} or actor-critic \cite{konda2003onactor,kumar2019sample}, whereas $Q$ learning is a standalone procedure. Other recent work focuses on policy search, a form of stochastic gradient with respect to a parameterized family of policies \cite{zhang2019global,8692920}, which is categorically different from fixed point iterations derived from Bellman's equations \cite{Bellman:1957}.}



==> Problem.tex <==
%!TEX root = root.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%  S  E  C  T  I  O  N    %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\section{Problem Formulation}\label{sec:prob}
\section{Policy Evaluation}\label{subsec:opt}%\vspace{-2mm}
%\blue{connective tissue}
We reformulate the fixed point problem \eqref{eq:bellman_operator_v} defined by Bellman's equation so that it may be identified with a nested stochastic program. {Since the resulting domain of this problem is intractable, we hypothesize that the Bellman fixed point belongs to a RKHS. Then, to apply the Representer Theorem, we require the introduction of regularization.}

We proceed with reformulating \eqref{eq:bellman_operator_v}: subtract the value function $V^{\pi}(\bbx)$ that satisfies the fixed point relation from both sides, and then pull it inside the expectation:
%
\begin{equation}\label{eq:bellman_operator_v_reformulate1}
0 = \mathbb{E}_{\bby}[ r(\bbx,\pi(\bbx),\bby) + \gamma V^{\pi}(\bby) -  V^{\pi} (\bbx)    \given \bbx, \pi(\bbx)]
\end{equation} 
%%
for all $\bbx \in \ccalX$. Value functions satisfying \eqref{eq:bellman_operator_v_reformulate1} are equivalent to those which satisfy the quadratic expression
%
%\begin{equation}\label{eq:bellman_operator_v_reformulate2}
$0=\frac{1}{2}( \mathbb{E}_{\bby}[ r(\bbx,\pi(\bbx),\bby) + \gamma V^{\pi}(\bby) -  V^{\pi}(\bbx)    \given \bbx, \pi(\bbx)])^2 \; ,$
%\end{equation} 
%%
which is null for all $\bbx \in \ccalX$, the starting point of the trajectory defining the value function \eqref{eq:value_function}. {To solve this expression for every $\bbx$, rather than solving it for a fixed $\bbx$ separately, we may integrate it out, which we do together with integrating over policy $\pi(\bbx)$ to yield the compositional stochastic program:}
%
\begin{align}
\label{eq:main_prob_0}
&V^{\pi} = \argmin_{V \in \ccalB(\ccalX)} J(V)  \\
&:= \!\argmin_{V \in \ccalB(\ccalX)} \mathbb{E}_{\bbx, \pi(\!\bbx\!)}\! \big\{\! \frac{1}{2}\!( \mathbb{E}_{\bby}\![ r(\bbx,\!\pi(\bbx\!)\!,\!\bby\!) \!\!+\! \gamma V\!(\bby\!) \!\!-\!\!  V \!(\!\bbx\!) \! \! \given\! \bbx,\! \pi(\!\bbx\!)])^2 \!\big\} \nonumber
\end{align}
%%
whose solutions coincide exactly with the fixed points of \eqref{eq:bellman_operator_v}. The equivalence of  \eqref{eq:bellman_operator_v_reformulate1} and \eqref{eq:main_prob_0} is not in general true, but only true when the probability distribution $\mu$ over $\bbx$ is ergodic. That is, for fixed policy $\pi$, $\mu$ is non-vanishing over the entire state space $\ccalX$: for each $\bbx \in \ccalX$, $\mu(\bbx) > 0$. Henceforth, we require $\mu$, the prior distribution over states $\bbx\in\ccalX$, to be ergodic. {See \cite{bhatnagar2009convergent,sutton2009fast} for a discussions of transforming Bellman equations into objective functions, and the necessity of ergodicity.}

 \eqref{eq:main_prob_0} defines a functional optimization problem which is intractable when we search over all bounded continuous functions $\ccalB(\ccalX)${. However, when} we restrict $\ccalB(\ccalX)$ to a Hilbert space $\ccalH$ equipped with a unique \emph{reproducing kernel}, i.e., an inner product-like map $\kappa: \ccalX \times \ccalX \rightarrow \reals$ {such that for $f\in\ccalH$,}%\vspace{-2mm}
%
\begin{align} \label{eq:rkhs_properties}
(i) \  \langle f , \kappa(\bbx, \cdot) \rangle _{\ccalH} \! = \! f(\bbx) \ % \text{for all } \bbx \in \ccalX , \nonumber\\
(ii) \ \ccalH = \closure{\text{span}\{ \kappa(\bbx , \cdot) \}} \; ,
\end{align}
 %
 %\blue{discussion of empirical vs. expected risk, what is $\bbx_n$, etc.}
for all $\bbx \in \ccalX$. We may apply the Representer Theorem to transform \eqref{eq:main_prob_0} into a semi-parametric one \cite{kimeldorf1971some,norkin2009stochastic}. In a RKHS, the optimal function $f\in\ccalH$ of \eqref{eq:main_prob_0} then takes the form \vspace{-1.5mm}
%
\begin{equation}\label{eq:kernel_expansion}
f(\bbx) = \sum_{n=1}^N w_n \kappa(\bbx_n, \bbx)\; {,}%%\vspace{-1mm}
\end{equation}
%
{where $\bbx_n$ is} a realization of {the} random variable $\bbx$. Thus, $f\in\ccalH$ is a kernel expansion \emph{only} at training samples. We define the upper summand index $N$  in \eqref{eq:kernel_expansion} in the kernel expansion of $f \in \ccalH$ {as the} model order, {which here} coincides with the training sample size.  %We further assume that the kernel is positive semidefinite, i.e. $\kappa(\bbx, \bbx') \geq 0$ for all $\bbx, \bbx' \in \ccalX$. 
%
 Common kernel choices are {polynomials and radial basis  (Gaussian) functions}, i.e., $\kappa(\bbx,\bbx') = \left(\bbx^T\bbx'+b\right)^c $ and $\kappa(\bbx,\bbx') = \exp\{ -{\lVert \bbx - \bbx' \rVert_2^2}/{2c^2} \}$, respectively.
%
In \eqref{eq:rkhs_properties}, property (i) is called the reproducing property, which follows from Riesz Representation Theorem \cite{wheeden1977measure}. Replacing $f$ by $\kappa(\bbx' , \cdot) $  in \eqref{eq:rkhs_properties} (i) yields $ \langle \kappa(\bbx', \cdot) , \kappa(\bbx, \cdot) \rangle_{\ccalH} = \kappa(\bbx, \bbx')$, the origin of the term ``reproducing kernel."  Moreover, property \eqref{eq:rkhs_properties} (ii) states that functions $f\in\ccalH$ admit a basis expansion in terms of kernels  \eqref{eq:kernel_expansion}. 
%
Such spaces are {called reproducing kernel Hilbert spaces (RKHSs)}. {When the kernel is universal} \cite{micchelli2006universal}, e.g., a Gaussian, a continuous function over a compact set may be approximated uniformly by one in a RKHS.

Subsequently, we seek to solve {\eqref{eq:main_prob_0}} with $V \in \ccalH$, and independent and identically distributed samples $(\bbx_t, \pi(\bbx_t), \bby_t)$ from the triple $(\bbx, \pi(\bbx), \bby)$ are sequentially available, yielding%\vspace{-2mm}
%
\begin{align}\label{eq:main_prob}
&V^{*}=\argmin_{V \in \ccalH} \mathbb{E}_{\bbx, \pi(\bbx)}\Big\{\frac{1}{2}( \mathbb{E}_{\bby}[ r(\bbx,\pi(\bbx),\bby)  \\
& \qquad\qquad\qquad\quad  + V(\bby) -  V (\bbx)    \given \bbx, \pi(\bbx)])^2\Big\} + \frac{\lambda}{2} \| V\|_{\ccalH}^2\nonumber
\end{align} 
%%
Hereafter, define $L(V) :=  \mathbb{E}_{\bbx, \pi(\bbx)}\{\frac{1}{2}( \mathbb{E}_{\bby}[ r(\bbx,\pi(\bbx),\bby) + \gamma V(\bby) -  V (\bbx)    \given \bbx, \pi(\bbx)])^2\} $ and $J(V) = L(V) + (\lambda/2)\|V\|_{\ccalH}^2$. The regularization term $(\lambda/2)\|V\|_{\ccalH}^2$ in \eqref{eq:main_prob} is needed to apply the Representer Theorem \eqref{eq:kernel_expansion} \cite{kimeldorf1971some}. Thus, policy evaluation in infinite MDPs \eqref{eq:main_prob} is both a specialization of compositional stochastic programming \cite{wang2017stochastic} to an objective defined by dynamic programming, and a generalization to the case where the decision variable is not vector-valued but is instead a function.%\vspace{-3mm}




